CubiXMusashi: Fusion of Wire-Driven CubiX and Musculoskeletal Humanoid Musashi toward Unlimited Performance

Humanoids exhibit a wide variety in terms of joint configuration, actuators, and degrees of freedom, resulting in different achievable movements and tasks for each type. Particularly, musculoskeletal humanoids are developed to closely emulate human body structure and movement functions, consisting of a skeletal framework driven by numerous muscle actuators. The redundant arrangement of muscles relative to the skeletal degrees of freedom has been used to represent the flexible and complex body movements observed in humans. However, due to this flexible body and high degrees of freedom, modeling, simulation, and control become extremely challenging, limiting the feasible movements and tasks. In this study, we integrate the musculoskeletal humanoid Musashi with the wire-driven robot CubiX, capable of connecting to the environment, to form CubiXMusashi. This combination addresses the shortcomings of traditional musculoskeletal humanoids and enables movements beyond the capabilities of other humanoids. CubiXMusashi connects to the environment with wires and drives by winding them, successfully achieving movements such as pull-up, rising from a lying pose, and mid-air kicking, which are difficult for Musashi alone. This concept demonstrates that various humanoids, not limited to musculoskeletal humanoids, can mitigate their physical constraints and acquire new abilities by connecting to the environment and driving through wires.

==> preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag} % 古いコマンドやパッケージの利用を警告する
\usepackage[all, warning]{onlyamsmath} % amsmath が提供しない数式環境を使用した場合に警告
% for not arxiv
% \usepackage[dvipdfmx]{color}
% \usepackage[dvipdfmx,bookmarks=true,bookmarksnumbered=true,bookmarkstype=toc,%
%      colorlinks=true,%
%      linkcolor=black, %%追加20090108
%      citecolor=black, %%追加20090108
%      urlcolor=black, %%追加20090108
%      bookmarksopen=true,%しおりツリーをデフォルトで開く
% %     backref=page,%citeにどこで使っているか出るようになる
%      pdftitle=\PDFTITLE,%
%      pdfsubject=\PDFSUBJECT,%
%      pdfauthor=\PDFAUTHOR,%
%      pdfkeywords=\PDFKEYWORDS]{hyperref}
% %% \usepackage[dvipdfmx]{graphicx}
% \usepackage[dvips]{graphicx}
% \usepackage[dvipdfmx]{}

% for arxiv
\usepackage{hyperref}
\usepackage{color}
\usepackage{graphicx}

% \usepackage{jtygm}
\usepackage{url} % \url のために必要
%% \url{http://nile.ulis.ac.jp/~yuka/}
\usepackage{txfonts,mathptmx}

%%%% カスタマイズしたい場合は以下に書く

\newcommand{\TODO}[1]{\fbox{{\textbf TODO:}#1}}
\usepackage{layout}
\usepackage{wrapfig}

% \usepackage{pxjahyper}
% hypcap: figref, tabrefしたときにジャンプ先がキャプション部ではなく図の上になる
\usepackage[figure,figure*,table,table*]{hypcap}
% \usepackage{eclbkbox}
%% \usepackage[dvipdfmx]{graphicx}
% \usepackage[dvipdfmx]{}
\usepackage{url} % \url のために必要
%% \url{http://nile.ulis.ac.jp/~yuka/}
%\usepackage{html} % latex2html で 利用
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{amsmath}
\algblockdefx{FORP}{ENDFORP}[1]%
  {\textbf{for}#1 \textbf{do in parallel}}%
  {\textbf{end for}}
\algnewcommand{\algorithmicand}{\textbf{ and }}
\algnewcommand{\algorithmicor}{\textbf{ or }}
\algnewcommand{\OR}{\algorithmicor}
\algnewcommand{\AND}{\algorithmicand}
% \usepackage[subrefformat=parens]{subcaption}
% \captionsetup{compatibility=false} % http://www.yamamo10.jp/yamamoto/comp/latex/make_doc/insert_fig/
% \captionsetup[sub]{skip=4pt}

%% \newcommand{\tabref}[1]{{表~\ref{#1}}~}
%% \newcommand{\figref}[1]{{図~\ref{#1}}~}
%% \newcommand{\equref}[1]{{式(\ref{#1})}~}
\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\subsecref}[1]{Subsection \ref{#1}}
\newcommand{\tabref}[1]{{Table \ref{#1}}}
\newcommand{\figref}[1]{{Fig. \ref{#1}}}
%% \newcommand{\figref}[1]{\figurename\ref{fig:#1}}
\newcommand{\equref}[1]{{Eq. \ref{#1}}}
\newcommand{\algoref}[1]{{Alg. \ref{#1}}}
\newcommand{\enumref}[1]{{\ref{#1}}}
%% \renewcommand{\figurename}{Fig.}
%% \renewcommand{\tablename}{Table }

\newcommand{\switchlanguage}[2]{%
  \ifx\paperlanguage\empty%
  #1%
  \else%
  #2%
  \fi%
}

